Virgo: Cluster-level Matrix Unit Integration in GPUs for Scalability and Energy Efficiency

Modern GPUs incorporate specialized matrix units such as Tensor Cores to accelerate GEMM operations, which are central to deep learning workloads. However, existing matrix unit designs are tightly coupled to the SIMT core, restricting operation size due to register file capacity and bandwidth constraints. Such a limitation in scalability makes it difficult to simultaneously improve compute throughput and energy efficiency in GPUs. To address this challenge, we propose Virgo, a GPU microarchitecture that integrates dedicated matrix units at the SIMT core cluster level. By decoupling the matrix unit from the SIMT core, Virgo eliminates scalability constraints imposed by the core microarchitecture. Consequently, Virgo increases operation granularity at the hardware level, reducing energy overhead from core instruction processing. Physical disaggregation also enables a unified matrix unit design and offloading both operand and accumulator accesses from the register file, improving data reuse and energy efficiency. Furthermore, this disaggregation supports efficient concurrent execution of the SIMT core and matrix unit, optimizing mapping for fused DNN workloads. Our evaluations using synthesizable RTL demonstrate that Virgo achieves 67.3% and 24.2% reduction in on-chip active power consumption, compared to the baseline Ampere-style and Hopper-style core-coupled designs.

==> ae-template.tex <==
\appendix
\section{Artifact Appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

{\em Obligatory}

\subsection{Artifact check-list (meta-information)}

{\em Obligatory. Use just a few informal keywords in all fields applicable to your artifacts
and remove the rest. This information is needed to find appropriate reviewers and gradually 
unify artifact meta information in Digital Libraries.}

{\small
\begin{itemize}
  \item {\bf Algorithm: }
  \item {\bf Program: }
  \item {\bf Compilation: }
  \item {\bf Transformations: }
  \item {\bf Binary: }
  \item {\bf Model: }
  \item {\bf Data set: }
  \item {\bf Run-time environment: }
  \item {\bf Hardware: }
  \item {\bf Run-time state: }
  \item {\bf Execution: }
  \item {\bf Metrics: }
  \item {\bf Output: }
  \item {\bf Experiments: }
  \item {\bf How much disk space required (approximately)?: }
  \item {\bf How much time is needed to prepare workflow (approximately)?: }
  \item {\bf How much time is needed to complete experiments (approximately)?: }
  \item {\bf Publicly available?: }
  \item {\bf Code licenses (if publicly available)?: }
  \item {\bf Data licenses (if publicly available)?: }
  \item {\bf Workflow framework used?: }
  \item {\bf Archived (provide DOI)?: }
\end{itemize}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{How to access}

{\em Obligatory}

\subsubsection{Hardware dependencies}

\subsubsection{Software dependencies}

\subsubsection{Data sets}

\subsubsection{Models}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}

{\em Obligatory}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected results}

{\em Obligatory}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment customization}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Methodology}

Submission, reviewing and badging methodology:

\begin{itemize}
  \item \url{https://www.acm.org/publications/policies/artifact-review-badging}
  \item \url{http://cTuning.org/ae/submission-20201122.html}
  \item \url{http://cTuning.org/ae/reviewing-20201122.html}
\end{itemize}


==> changes.tex <==
We thank the reviewers for their thoughtful comments.
Please find below a description of the changes we made to the paper, as well as
the relevant sections for the changes.

\textbf{\\New Hopper Tensor Core Baseline}

\hll{Sections~{\ref{sec:method-hopper}} and {\ref{sec:eval-gemm}}}.

\begin{itemize}
\item{ We implemented a new baseline design that models NVIDIA Hopper's operand
decoupling mechanism.  With this addition, we comprehensively cover existing
integration methods of (1) Volta-style tightly-coupled, (2) Ampere-style DMA-integrated and (3)
Hopper-style operand-decoupled designs, as we clarify in \hll{Section
{\ref{sec:terminology}}. }}
\item{Although the Hopper baseline relieves register file constraints
by operand offloading, it is still limited by storing accumulator data
in the register file. This resulted in substantial energy consumption overhead of
32.5\% over Virgo.}
\item{
With this baseline, we model how an asynchronous design can benefit core-coupled
designs as well, which is the case for modern GPUs such as AMD MI300 and NVIDIA
Hopper.  The asynchronous interface does increase hardware utilization due to
being less constrained by core instruction throughput, albeit with the
power and data reuse disadvantages.
}
\item{
We find that due to being a core-coupled design, each Hopper-style matrix unit
in different cores need to make duplicated SMEM accesses and achieve suboptimal
data reuse, compared to the unified design that Virgo enables by physical
disaggregation (\hll{Table~{\ref{tab:smem-footprint}}}).
% memory, and writes accumulator data back to the register file.  Due to the
% partial decoupling, we find the Hopper-style baseline still encounters limited
% scalability, with the tile size limited to 16\texttimes16\texttimes32 and 64
% MACs per unit.
}
\end{itemize}

\textbf{\\Scaled-Up Tensor Core Baseline with FP16}

\hll{Section~{\ref{sec:eval-gemm}}}.

\begin{itemize}
\item{To further with modern designs, we scaled up our
Volta and Ampere-style Tensor Core baselines by adding FP16 support, doubling
the number of MACs within the same bandwidth.  Virgo's systolic array is also
scaled to 16x16.}
\item{This increases the Tensor-to-SIMT FLOPS ratio for the Volta/Ampere
baselines from 2:1 to 4:1, and Hopper-style baseline to 8:1, approaching
configurations seen in modern designs like MI300 or Ampere.
}
\end{itemize}

% Our results demonstrate a 1.66x speedup for Virgo over the scaled-up TC, alongside 63.9% active power
% savings (22.2% absolute power savings), consistent with the original results.

\textbf{\\FlashAttention-3 Application Study}

\hll{Sections {\ref{sec:flash-mapping}} and {\ref{sec:eval-flash}}}.

\begin{itemize}
\item{For a more sophisticated application-level study beyond GEMM, we
introduced a new experiment using the FlashAttention-3 kernel, which benefits
from Virgo's ability to schedule GEMM and softmax within a tile concurrently.}
\item{This workload demonstrates that efficient overlapping of matrix and SIMT
compute can be achieved with minimal synchronization overhead of 2.4\% of the
total runtime. \hll{Sections {\ref{sec:programming-sync-overhead}}}}
\item{This experiment also highlights an advantage of the disaggregated design,
which eliminates contentions to instruction slots and register ports between the
matrix and SIMT compute.}
\end{itemize}

\textbf{\\Benefits of Physical Disaggregation}

The new experiments data we add quantitatively demonstrates the following
benefits of disaggregated matrix unit design, over a Hopper-style operand-decoupled design:

\begin{enumerate}
\item{Scalability from larger tile sizes, by decoupling accumulator
data from the register file. \hll{Sections~{\ref{sec:method-hopper}} and {\ref{sec:gemm-power-energy}}}}
\item{Power and energy efficiency from eliminating redundant RF accesses
for the operand and accumulator data delivery. \hll{Section~{\ref{sec:gemm-power-energy}}}}
\item{Better data reuse in reduced energy consumption in the shared memory,
due to enabling a unified design at the cluster. \hll{Section~{\ref{sec:eval-smem-reuse}}}}\item{Efficient offloading of core pipeline resources to non-matrix compute,
eliminating contention for issue slots and register file ports. \hll{Section~{\ref{sec:eval-flash}}}}
\end{enumerate}

\textbf{\\Programming Model and Compiler/System Software Discussions}

% Discuss how compiler and/or system software support would need to change with disaggregation.
\begin{itemize}
\item{
We added \hll{Section~{\ref{sec:programming-api}}} to discuss how
Virgo's asynchronous primitives can be used to construct a higher-level API that
makes it easier for programmers to write full GEMM or fused kernels, along with
a code snippet that demonstrates this with FlashAttention-3.
}
\item{We also added a discussion on how code generation schemes in
domain-specific compiler frameworks such as Triton or JAX can be applied to
Virgo's programming primitives in \hll{Section~{\ref{sec:programming-codegen}}}.}
\end{itemize}

\textbf{\\Asynchronous vector/matrix co-execution in industry designs}

We augmented \hll{Section~{\ref{sec:programming-async}}} with a clarification
that the asynchronous design and single-warp co-execution of matrix units is
commonly found in recent industry designs.  
